Orbital maneuvers for a space probe around Titania

For most space missions, it is interesting that the probe remains for a considerable time around the mission target. The longer the lifetime of a mission, the greater the chances of collecting information about the orbited body. In this work, we present orbital maneuvers that aim to show how to avoid a collision of a space probe with the surface of Titania. Through an expansion of the gravitational potential to the second order, the asymmetry of the gravitational field due to the coefficient $C_{22}$ of Titania, the zonal coefficient $J_2$, and the gravitational perturbation of Uranus are considered. Two models of coplanar bi-impulse maneuvers are presented. The first maneuver consists of transferring an initial elliptical orbit to a final circular orbit, and the second has the objective of transferring an initial elliptical orbit to a final orbit that is also elliptical. The lag in the inclination and semi-major axis of the orbits is investigated before performing the maneuvers. To point out the best scenarios for carrying out the maneuvers, a study is presented for different points of an orbit where transfers could be made. In addition, a maneuver strategy is presented to correct the variation of the periapsis argument. The results show that maneuvers performed a few days after integration are more economical than maneuvers performed later, a few days before the collision. The economy of the maneuvers is also demonstrated through an analysis of the ratio of the increase in speed to the lifetime.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} Hofstadter, Uranus and Neptune missions: A study in advance of the next Planetary Science Decadal Survey. Planetary and Space Science 2019.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


